ACORN: Performant and Predicate-Agnostic Search Over Vector Embeddings and Structured Data

Applications increasingly leverage mixed-modality data, and must jointly search over vector data, such as embedded images, text and video, as well as structured data, such as attributes and keywords. Proposed methods for this hybrid search setting either suffer from poor performance or support a severely restricted set of search predicates (e.g., only small sets of equality predicates), making them impractical for many applications. To address this, we present ACORN, an approach for performant and predicate-agnostic hybrid search. ACORN builds on Hierarchical Navigable Small Worlds (HNSW), a state-of-the-art graph-based approximate nearest neighbor index, and can be implemented efficiently by extending existing HNSW libraries. ACORN introduces the idea of predicate subgraph traversal to emulate a theoretically ideal, but impractical, hybrid search strategy. ACORN's predicate-agnostic construction algorithm is designed to enable this effective search strategy, while supporting a wide array of predicate sets and query semantics. We systematically evaluate ACORN on both prior benchmark datasets, with simple, low-cardinality predicate sets, and complex multi-modal datasets not supported by prior methods. We show that ACORN achieves state-of-the-art performance on all datasets, outperforming prior methods with 2-1,000x higher throughput at a fixed recall.

==> algs/ACORN-ann-search.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets

% \begin{algorithm}[hbt!]
\begin{algorithm}[hbt!]
\caption{ACORN-ANN-SEARCH($x_q, p_q, K, efs$)}\label{alg:acorn-ann-search}
\KwIn{query vector $x_q$, query predicate $p_q$, number of nearest neighbors to return $K$, size of dynamic candidate list $efs$}
\KwOut{$K$ nearest elements to $x_q$}
$ep \gets$ entry-point to graph\\
$W \gets \emptyset$ \Comment{set of current nearest}\
$L \gets level(ep)$ \Comment{uppermost level}\ 
\For{$l \gets L...1$}{
    $ep \gets$ SEARCH-LAYER($x_q, p_q, ep, ef=1, l$)\
  }\
$W \gets$ SEARCH-LAYER($x_q, p_q, ep, ef=efs, l=0$)\

\Return{$K$ nearest elements from $W$ to $x_q$}\
\end{algorithm}

% Some notes: search layer on the upper levels matches to faiss hnsw::greedy\_update\_nearest and on level 0 corresponds to hsnw::search\_from\_candidates. This is exactly smae as HNSW alg except for the added predicate $p_q$


==> algs/ACORN-find-candidates.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets


% \begin{algorithm}[hbt!]
\begin{algorithm}[hbt!]
\caption{ACORN-FIND-CANDIDATES($x_q, ep, ef, l$)}\label{alg:acorn-find candidates}
\KwIn{query vector $q$, query predicate $p_q$, entry-point $ep$, number of nearest neighbors to return $ef$,  level to search $l$}
\KwOut{$ef$ nearest elements to $x_q$}
$T \gets ep$ \Comment{visited set}\
$C \gets ep$ \Comment{candidate set}\
$W \gets ep$ \Comment{dynamic list of found nearest neighbors}\
$max\_size \gets M \times \gamma$ \Comment{determined by index construction parameters}\

\While{$|C| > 0$}{
    $c \gets$ extract $\argmin_{x\in C} \lVert x_q - x\rVert$ \\
    $f \gets$ get $\argmax_{x\in W} \lVert x_q - x\rVert$ \\
    % $c \gets$ pop nearest element from $C$ to $x_q$\\
    % $f \gets$ get farthest element from $W$ to $x_q$\\
    \uIf{$|W| >= max\_size$} {
        break
    }
    $neighborhood \gets$ GET-NEIGHBORS-SIMPLE($c, l$)\\
    % \ForEach{$v\in N^l(c)$}{
    \ForEach{$v\in$ neighborhood$[1{:}M]$}{
        \uIf{$v\notin T$}{
            $T\gets T\cup v$\\
            $f \gets \argmax_{x\in W} \lVert x_q - x\rVert$ \\
            % $f \gets$ get farthest element from $W$ to $x_q$\\               
            \uIf{$dist(v, x_q) < dist(f, x_q)$ or $|W| < ef$}{
                $C \gets C\cup v$\\
                $W \gets W \cup v$\\
                \uIf{$|W| > ef$} {
                    remove furthest element from $W$ to $x_q$
                }   
            }
        }
    }\
    

}
\Return{$W$}\
\end{algorithm}

% Some notes: the main difference between this function and SEARCH-LAYER is that here, i) we don't use a greedy break, instead we break if we've found the desired (M*gamma) number of nodes, ii) Also the GET-NEIGHBORS function is the simple version iii) lastly, the $p_q$ is not a parameter since the construction alg is metadata agnostic, while search is not. This function corresponds to HybridHNSW's search\_neighbors\_to\_add (can probably collapse this into ACORN-SEARCH-LAYER)

==> algs/ACORN-get-neighbors.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets


\begin{algorithm}[hbt!]
\caption{GET-NEIGHBORS-SIMPLE($v, l$)}\label{alg:acorn-get-neighbors-simple}
\KwIn{node $v$, level $l$ to select neighbors from}
\KwOut{neighbor list of $x_q$}
$R \gets N^l(v)$ \Comment{neighbor list to return}\
\Return{$R$}\
\end{algorithm}

% \begin{algorithm}[hbt!]
\begin{algorithm}[hbt!]
\caption{GET-NEIGHBORS-FILTER($v, l, p_q$)}\label{alg:acorn-get-neighbors-filter}
\KwIn{node $v$, level $l$ to select neighbors from, query predicate $p_q$}
\KwOut{neighbor list of $x_q$}
$R \gets \emptyset$ \Comment{neighbor list to return}\
\ForEach{$u\in N^l(v)$}{
    \uIf{$u \passes p_q$} {
        $R \gets R\cup u$
    }
}
\Return{$R$}\
\end{algorithm}


\begin{algorithm}[hbt!]
\caption{GET-NEIGHBORS-HEURISTIC($v, l, p_q$)}\label{alg:acorn-get-neighbors-heuristic}
\KwIn{node $v$, level $l$ to select neighbors from, query predicate $p_q$}
\KwOut{neighbor list of $x_q$}
$M_{\beta} \gets$ graph parameter $M_{\beta}$\\
$R \gets \emptyset$ \Comment{neighbor list to return}\
\ForEach{$u\in N^l(v)[1{:}M_{\beta}]$}{
    \uIf{$u \passes p_q$} {
        $R \gets R\cup u$
    }
}
\ForEach{$u\in N^{l}(v)[{M_{\beta}+1{:}}]$}{
    \uIf{$u \passes p_q$} {
        $R \gets R\cup u$
    }
    \ForEach{$y\in N^{l}(v)$}  {
        \uIf{$y \passes p_q$} {
            $R \gets R\cup y$
        }
    }
}
\Return{$R$}\
\end{algorithm}

\begin{algorithm}[hbt!]
\caption{GET-NEIGHBORS-EXPANSION($v, l, p_q$)}\label{alg:acorn-get-neighbors-expansion}
\KwIn{node $v$, level $l$ to select neighbors from, query predicate $p_q$}
\KwOut{neighbor list of $x_q$}
$R \gets \emptyset$ \Comment{neighbor list to return}\
\ForEach{$u\in N^{l}(v)$}{
    \uIf{$u \passes p_q$} {
        $R \gets R\cup u$
    }
    \ForEach{$y\in N^{l}(v)$}  {
        \uIf{$y \passes p_q$} {
            $R \gets R\cup y$
        }
    }
}
\Return{$R$}\
\end{algorithm}

% Some notes: when $M_{\beta} \geq M*2*\gamma$, this corresponds to the simple strategy. GET-NEIGHBORS-SIMPLE is used for upper levels, while the GET-NEIGHBORS-ACORN is used for bottom level. GET-NEIGHBORS-EXPANSION is used for ACORN-HNSW search

==> algs/ACORN-prune.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets


% \begin{algorithm}[hbt!]
\begin{algorithm}[hbt!]
\caption{ACORN-PRUNE($x_q, C, M_{\beta}, l$)}\label{alg:acorn-prune}
\KwIn{base element $x_q$, candidate neighbors $C$, compression parameter $M_{\beta}$, level $l$}
\KwOut{selected neighbors for $x_q$ from $C$}
$R \gets \emptyset$\\
$H \gets \emptyset$ \Comment{2-hop neighbor set}\
max\_size $\gets M\times\gamma$\\
\For{$i = 0;\ i < M_\beta;\ i++$}{
    $c \gets$ extract from $C$ $\argmin_{x\in C} \lVert x_q - x\rVert$ \\
    $R \gets R\cup c$\\
    break if $|R| >$ max\_size
}
\While{$|C| > 0$}{
    $c \gets$ extract from $C$ $\argmin_{x\in C} \lVert x_q - x\rVert$ \\
    \uIf{$c \not\in H$}{
        $R \gets R \cup c$\\
        $H \gets H \cup N^l(c)$\\
       
    }
    break if $|H| >$ max\_size
   
}


\Return{$R$}\
\end{algorithm}

% Some notes: this corresponds to HybridHNSW shrink\_neighbor\_list with pruningFlag 0 in faiss implementation. 


==> algs/ACORN_insert.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets



% \begin{algorithm}[hbt!]
\begin{algorithm}[hbt!]
\caption{ACORN-INSERT($x_q, M, efc, \gamma, M_{\beta}$)}\label{alg:acorn-insert}
\KwIn{new element $x_q$, maximum number of neighbors to find for each element per level during search,  size of dynmic candidate list $efc$, neighbor expansion factor $\gamma$, edge list compression parameter $M_{\beta}$}
\KwOut{updated hnsw graph with $x_q$ inserted}
$W \gets \emptyset$ \Comment{set of currently found nearest elements}\
$ep \gets$ entry-point to graph\\
$L \gets level(ep)$ \Comment{Top graph level}\ 
$m_L \gets 1/ln(M)$\\
$l_q \gets \lfloor -ln(unif(0..1))\times m_L \rfloor$ \Comment{level assignment for $x_q$}
\For{$l \gets L ... l_q+1$}{
    $ep \gets$ ACORN-SEARCH-LAYER($x_q, p_q=*, ep, ef=1, l$)\\
  }\
\For{$l \gets \min(L, l_q)...0$}{
    % $W \gets$ ACORN-FIND-CANDIDATES($x_q, ep, efc\times\gamma, l$)\\
    $W \gets$ ACORN-SEARCH-LAYER($x_q, p_q = *, ep, efc\times\gamma, l$)\\
    $neighbors \gets W$\\
    \uIf{l = 0}{
        $neighbors\gets$ ACORN-PRUNE($x_q, W, M, l$)\\
    } 
    
    \ForEach{$v\in neighbors$} {
        add bidirectional edges between $v$ and $x_q$\\
        \uIf{$|N^{l}(v)| > M \times \gamma $} {
            shrink neighbor list to size $M\times \gamma$\\
            \uIf{l = 0}{
                $neighbors\gets$ ACORN-PRUNE($v, N^l(v), M, l$)\\
            } 
        }
    
    }
    $ep \gets W$\\
  }\
\If{$l_q > L$} {
    update graph entrypoint to $x_q$
}

\end{algorithm}

% Some notes: This function corresponds to faiss::add\_links\_starting\_from in the HybridHNSW implementation. SEARCH-LAYER uses GET-NEIGHBORS-SIMPLE. $m_L = 1/ln(M)$. HNSW also uses M for upper levels and 2M as maximum number of neighbors on level 0, but we'll ignore this for simplicity. 


==> algs/hnsw-search-layer.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets


% \begin{algorithm}[hbt!]
\begin{algorithm}[H]
\caption{HNSW-SEARCH-LAYER($x_q, ep, ef, l$)}\label{alg:hnsw-search-layer}
\KwIn{query vector $q$, entry-point $ep$, number of nearest neighbors to return $ef$,  level to search $l$}
\KwOut{$ef$ nearest elements to $x_q$}
$T \gets ep$ \Comment{visited set}
$C \gets ep$ \Comment{candidate set}
$W \gets ep$ \Comment{dynamic list of found nearest neighbors}

\While{$|C| > 0$}{
    $c \gets$ extracts $\argmin_{x\in C} \lVert x_q - x\rVert$ \\
    $f \gets$ get $\argmax_{x\in W} \lVert x_q - x\rVert$ \\
    % $c \gets$ pop nearest element from $C$ to $x_q$\\
    % $f \gets$ get farthest element from $W$ to $x_q$\\
    \uIf{$dist(c, q) > dist(f, q)$} {
        break
    }
    \ForEach{$v\in N^l(c)$}{
        \uIf{$v\notin T$}{
            $T\gets T\cup v$\\
            $f \gets \argmax_{x\in W} \lVert x_q - x\rVert$ \\
            % $f \gets$ get farthest element from $W$ to $x_q$\\               
            \uIf{$dist(v, x_q) < dist(f, x_q)$ or $|W| < ef$}{
                $C \gets C\cup v$\\
                $W \gets W \cup v$\\
                \uIf{$|W| > ef$} {
                    remove furthest element from $W$ to $x_q$
                }   
            }
        }
    }\
    

}


\Return{$W$}\
\end{algorithm}

Some notes: search layer on the upper levels matches to faiss hnsw::greedy\_update\_nearest and on level 0 corresponds to hsnw::search\_from\_candidates. In hybrid construction, we look at only the beginning of each neighborhood. Notation $N^l(v)$ represents v's neighborhood at level $l$

==> algs/hnsw_insert.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets



% \begin{algorithm}[hbt!]
\begin{algorithm}[H]
\caption{HNSW-INSERT($x_q, M, efc$)}\label{alg:hnsw-insert}
\KwIn{new element $x_q$, maximum number of neighbors for each element per level M,  size of dynmic candidate list $efc$}
\KwOut{updated hnsw graph with $x_q$ inserted}
$W \gets \emptyset$ \Comment{set of currently found nearest elements}\
$ep \gets$ entry-point to hnsw graph\\
$L \gets level(ep)$ \Comment{Top hnsw level}\ 
$m_L \gets 1/ln(M)$\\
$l_q \gets \lfloor -ln(unif(0..1))\times m_L \rfloor$ \Comment{level assignment for $x_q$}
\For{$l \gets L ... l_q+1$}{
    $ep \gets$ SEARCH-LAYER($x_q, ep, ef=1, l$)\\
  }\
\For{$l \gets \min(L, l_q)...0$}{
    $W \gets$ SEARCH-LAYER($x_q, ep, efc, l$)\\
    $neighbors\gets$ HNSW-PRUNE($x_q, W, M, l$)\\
    \ForEach{$v\in neighbors$} {
        add bidirectional edges between $v$ and $x_q$\\
        \uIf{$|N^{l}(v)| > M_l$} {
            $N^{l}(v) \gets$ HNSW-PRUNE($v, N^{l}(v), M_l, l$)
        }
    
    }
    $ep \gets W$\\
  }\
\If{$l_q > L$} {
    update hnsw entrypoint to $x_q$
}

\end{algorithm}

Some notes: $m_L = 1/ln(M)$. HNSW also uses M for upper levels and 2M as maximum number of neighbors on level 0, but we'll ignore this for simplicity. Note also that faiss implementation doesn't update the entrypoint on the levels at $l_q$ and below for some strange reason - this could cause slower than necessary construction (?)


==> algs/hnsw_prune.tex <==
%% This is needed if you want to add comments in
%% your algorithm with \Comment
\RestyleAlgo{ruled}

% \DontPrintSemicolon

\SetKwComment{Comment}{// }{} %can chage the comment format by changing text in brackets


% \begin{algorithm}[hbt!]
\begin{algorithm}[H]
\caption{HNSW-PRUNE($x_q, C, M, $)}\label{alg:hnsw-prune}
\KwIn{base element $x_q$, candidate neighbors $C$, max number of neighbors to return $M$}
\KwOut{at most $M$ selected neighbors for $x_q$ from $C$}
$R \gets \emptyset$\\

\While{$|C| > 0$ and $|R| < M$}{
    $c \gets$ extract from $C$ $\argmin_{x\in C} \lVert x_q - x\rVert$ \\
    \uIf{$dist(x_q, c) < \min_{x\in R} dist(c, x)$}{
        $R \gets R \cup c$\\
    }
}


\Return{$R$}\
\end{algorithm}

Some notes: search layer on the upper levels matches to faiss hnsw::greedy\_update\_nearest and on level 0 corresponds to hsnw::search\_from\_candidates. In hybrid construction, we look at only the beginning of each neighborhood

